Exploring the Nature of Little Red Dots: Constraints on AGN and Stellar Contributions from PRIMER MIRI Imaging

JWST has revealed a large population of compact, red galaxies at $z>4$ known as Little Red Dots (LRDs). We analyze the spectral energy distributions (SEDs) of 95 LRDs from the JWST PRIMER survey with complete photometric coverage from $1-18\ \mu$m using NIRCam and MIRI imaging, representing the most extensive SED analysis on a large LRD sample with long-wavelength MIRI data. We examine SED models in which either galaxy or active galactic nucleus (AGN) emission dominates the rest-frame UV or optical continuum, extracting physical properties to explore each scenario's implications. In the galaxy-only model, we find massive, dusty stellar populations alongside unobscured, low-mass components, hinting at inhomogeneous obscuration. The AGN-only model indicates dusty, luminous AGNs with low hot dust fractions compared to typical quasars. A hybrid AGN and galaxy model suggests low-mass, unobscured galaxies in the UV, with stellar mass estimates spanning $\sim$2 dex across the different models, underscoring the need for caution in interpreting LRD stellar masses. With MIRI photometry, the galaxy-only model produces stellar masses within cosmological limits, but extremely high stellar mass densities are inferred. The hybrid model infers highly overmassive black holes exceeding those in recently reported high-redshift AGNs, hinting at a partial AGN contribution to the rest-optical continuum or widespread super-Eddington accretion. Our findings highlight the extreme conditions required for both AGN or galaxy dominated scenarios in LRDs, supporting a mixed contribution to the red continuum, or novel scenarios to explain the observed emission.

==> figset.tex <==
\figsetstart
\figsetnum{3}
\figsettitle{Images}

\figsetgrpstart
\figsetgrpnum{3.1}
\figsetgrptitle{COSMOS 2144.}
\figsetplot{cosmos_2144_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.2}
\figsetgrptitle{COSMOS 2356.}
\figsetplot{cosmos_2356_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.3}
\figsetgrptitle{COSMOS 2451.}
\figsetplot{cosmos_2451_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.4}
\figsetgrptitle{COSMOS 5229.}
\figsetplot{cosmos_5229_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.5}
\figsetgrptitle{COSMOS 5621.}
\figsetplot{cosmos_5621_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.6}
\figsetgrptitle{COSMOS 5844.}
\figsetplot{cosmos_5844_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.7}
\figsetgrptitle{COSMOS 7071.}
\figsetplot{cosmos_7071_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.8}
\figsetgrptitle{COSMOS 7236.}
\figsetplot{cosmos_7236_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.9}
\figsetgrptitle{COSMOS 8227.}
\figsetplot{cosmos_8227_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.10}
\figsetgrptitle{COSMOS 8406.}
\figsetplot{cosmos_8406_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.11}
\figsetgrptitle{COSMOS 8550.}
\figsetplot{cosmos_8550_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.12}
\figsetgrptitle{COSMOS 11625.}
\figsetplot{cosmos_11625_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.13}
\figsetgrptitle{COSMOS 12184.}
\figsetplot{cosmos_12184_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.14}
\figsetgrptitle{COSMOS 13104.}
\figsetplot{cosmos_13104_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.15}
\figsetgrptitle{COSMOS 13886.}
\figsetplot{cosmos_13886_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.16}
\figsetgrptitle{COSMOS 15702.}
\figsetplot{cosmos_15702_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.17}
\figsetgrptitle{COSMOS 18805.}
\figsetplot{cosmos_18805_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.18}
\figsetgrptitle{COSMOS 20188.}
\figsetplot{cosmos_20188_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.19}
\figsetgrptitle{COSMOS 20492.}
\figsetplot{cosmos_20492_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.20}
\figsetgrptitle{COSMOS 20652.}
\figsetplot{cosmos_20652_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.21}
\figsetgrptitle{COSMOS 21273.}
\figsetplot{cosmos_21273_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.22}
\figsetgrptitle{COSMOS 21309.}
\figsetplot{cosmos_21309_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.23}
\figsetgrptitle{COSMOS 22424.}
\figsetplot{cosmos_22424_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.24}
\figsetgrptitle{COSMOS 22433.}
\figsetplot{cosmos_22433_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.25}
\figsetgrptitle{COSMOS 25273.}
\figsetplot{cosmos_25273_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.26}
\figsetgrptitle{COSMOS 26016.}
\figsetplot{cosmos_26016_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.27}
\figsetgrptitle{COSMOS 26234.}
\figsetplot{cosmos_26234_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.28}
\figsetgrptitle{COSMOS 26676.}
\figsetplot{cosmos_26676_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.29}
\figsetgrptitle{COSMOS 27477.}
\figsetplot{cosmos_27477_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.30}
\figsetgrptitle{COSMOS 30244.}
\figsetplot{cosmos_30244_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.31}
\figsetgrptitle{COSMOS 35781.}
\figsetplot{cosmos_35781_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.32}
\figsetgrptitle{COSMOS 67746.}
\figsetplot{cosmos_67746_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.33}
\figsetgrptitle{COSMOS 74251.}
\figsetplot{cosmos_74251_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.34}
\figsetgrptitle{COSMOS 75330.}
\figsetplot{cosmos_75330_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.35}
\figsetgrptitle{COSMOS 79014.}
\figsetplot{cosmos_79014_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.36}
\figsetgrptitle{COSMOS 108622.}
\figsetplot{cosmos_108622_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.37}
\figsetgrptitle{COSMOS 111762.}
\figsetplot{cosmos_111762_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.38}
\figsetgrptitle{UDS 4090.}
\figsetplot{uds_4090_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.39}
\figsetgrptitle{UDS 4396.}
\figsetplot{uds_4396_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.40}
\figsetgrptitle{UDS 4828.}
\figsetplot{uds_4828_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.41}
\figsetgrptitle{UDS 5280.}
\figsetplot{uds_5280_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.42}
\figsetgrptitle{UDS 5480.}
\figsetplot{uds_5480_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.43}
\figsetgrptitle{UDS 5719.}
\figsetplot{uds_5719_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.44}
\figsetgrptitle{UDS 6563.}
\figsetplot{uds_6563_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.45}
\figsetgrptitle{UDS 9235.}
\figsetplot{uds_9235_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.46}
\figsetgrptitle{UDS 10330.}
\figsetplot{uds_10330_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.47}
\figsetgrptitle{UDS 13468.}
\figsetplot{uds_13468_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.48}
\figsetgrptitle{UDS 13624.}
\figsetplot{uds_13624_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.49}
\figsetgrptitle{UDS 13932.}
\figsetplot{uds_13932_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.50}
\figsetgrptitle{UDS 14126.}
\figsetplot{uds_14126_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.51}
\figsetgrptitle{UDS 14305.}
\figsetplot{uds_14305_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.52}
\figsetgrptitle{UDS 14388.}
\figsetplot{uds_14388_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.53}
\figsetgrptitle{UDS 15912.}
\figsetplot{uds_15912_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.54}
\figsetgrptitle{UDS 17160.}
\figsetplot{uds_17160_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.55}
\figsetgrptitle{UDS 17818.}
\figsetplot{uds_17818_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.56}
\figsetgrptitle{UDS 33438.}
\figsetplot{uds_33438_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.57}
\figsetgrptitle{UDS 34633.}
\figsetplot{uds_34633_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.58}
\figsetgrptitle{UDS 34737.}
\figsetplot{uds_34737_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.59}
\figsetgrptitle{UDS 34815.}
\figsetplot{uds_34815_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.60}
\figsetgrptitle{UDS 34899.}
\figsetplot{uds_34899_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.61}
\figsetgrptitle{UDS 35121.}
\figsetplot{uds_35121_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.62}
\figsetgrptitle{UDS 38096.}
\figsetplot{uds_38096_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.63}
\figsetgrptitle{UDS 39469.}
\figsetplot{uds_39469_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.64}
\figsetgrptitle{UDS 40579.}
\figsetplot{uds_40579_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.65}
\figsetgrptitle{UDS 40898.}
\figsetplot{uds_40898_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.66}
\figsetgrptitle{UDS 41039.}
\figsetplot{uds_41039_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.67}
\figsetgrptitle{UDS 44702.}
\figsetplot{uds_44702_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.68}
\figsetgrptitle{UDS 44877.}
\figsetplot{uds_44877_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.69}
\figsetgrptitle{UDS 46014.}
\figsetplot{uds_46014_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.70}
\figsetgrptitle{UDS 60251.}
\figsetplot{uds_60251_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.71}
\figsetgrptitle{UDS 62612.}
\figsetplot{uds_62612_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.72}
\figsetgrptitle{UDS 66751.}
\figsetplot{uds_66751_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.73}
\figsetgrptitle{UDS 68913.}
\figsetplot{uds_68913_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.74}
\figsetgrptitle{UDS 75424.}
\figsetplot{uds_75424_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.75}
\figsetgrptitle{UDS 76730.}
\figsetplot{uds_76730_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.76}
\figsetgrptitle{UDS 77750.}
\figsetplot{uds_77750_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.77}
\figsetgrptitle{UDS 78549.}
\figsetplot{uds_78549_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.78}
\figsetgrptitle{UDS 81578.}
\figsetplot{uds_81578_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.79}
\figsetgrptitle{UDS 81866.}
\figsetplot{uds_81866_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.80}
\figsetgrptitle{UDS 84401.}
\figsetplot{uds_84401_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.81}
\figsetgrptitle{UDS 144265.}
\figsetplot{uds_144265_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.82}
\figsetgrptitle{UDS 149541.}
\figsetplot{uds_149541_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.83}
\figsetgrptitle{UDS 151980.}
\figsetplot{uds_151980_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.84}
\figsetgrptitle{UDS 152026.}
\figsetplot{uds_152026_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.85}
\figsetgrptitle{UDS 152826.}
\figsetplot{uds_152826_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.86}
\figsetgrptitle{UDS 153498.}
\figsetplot{uds_153498_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.87}
\figsetgrptitle{UDS 159206.}
\figsetplot{uds_159206_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.88}
\figsetgrptitle{UDS 161988.}
\figsetplot{uds_161988_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.89}
\figsetgrptitle{UDS 165865.}
\figsetplot{uds_165865_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.90}
\figsetgrptitle{UDS 170710.}
\figsetplot{uds_170710_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.91}
\figsetgrptitle{UDS 173887.}
\figsetplot{uds_173887_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.92}
\figsetgrptitle{UDS 177350.}
\figsetplot{uds_177350_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.93}
\figsetgrptitle{UDS 178738.}
\figsetplot{uds_178738_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.94}
\figsetgrptitle{UDS 181563.}
\figsetplot{uds_181563_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{3.95}
\figsetgrptitle{UDS 183087.}
\figsetplot{uds_183087_sed.pdf}
\figsetgrpnote{Image cutout and SED of the LRD. The top panel shows 2'' stamp images. The bottom panel shows the observed photometry in the black points, and $2\sigma$ upper limits for non-detections, except for F1800W, where $5\sigma$ upper limits are shown for non-detections. The median (colored lines) and 68\% posterior (shaded regions) of the galaxy-only, AGN-only and hybrid models are shown from left to right. The rest-UV stellar component is shown in blue, rest-optical stellar component in orange, reddened accretion disk emission in red, scattered accretion disk in green, and hot dust emission in violet.}
\figsetgrpend

\figsetend
